Understanding Intrinsic Socioeconomic Biases in Large Language Models

Large Language Models (LLMs) are increasingly integrated into critical decision-making processes, such as loan approvals and visa applications, where inherent biases can lead to discriminatory outcomes. In this paper, we examine the nuanced relationship between demographic attributes and socioeconomic biases in LLMs, a crucial yet understudied area of fairness in LLMs. We introduce a novel dataset of one million English sentences to systematically quantify socioeconomic biases across various demographic groups. Our findings reveal pervasive socioeconomic biases in both established models such as GPT-2 and state-of-the-art models like Llama 2 and Falcon. We demonstrate that these biases are significantly amplified when considering intersectionality, with LLMs exhibiting a remarkable capacity to extract multiple demographic attributes from names and then correlate them with specific socioeconomic biases. This research highlights the urgent necessity for proactive and robust bias mitigation techniques to safeguard against discriminatory outcomes when deploying these powerful models in critical real-world applications.

==> figure_scripts/fig_arbitrariness_spread.tex <==
\begin{tikzpicture}
\begin{axis} [width=0.37\linewidth,height=0.25\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ylabel={\% of Data Points},ymin=0,ymax=25,xmin=0.525,xmax=0.975,xlabel={Self-Consistency (CDF)},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm, font=\small},xlabel style={align=center, text width=4cm, font=\small},
xtick={0.5, 0.6, 0.7, 0.8, 0.9, 1.},ticklabel style = {font=\small},
% legend pos=north west, legend columns=2,legend style={font=\small,at={(0.5,-0.4)},anchor=north}, 
title style={align=center, text width=5cm, font=\small},
title={\textbf{\vphantom{g}(a) Cumulative Distribution of Multiplicity}}
]

\addplot [rwhite,ultra thick] table[x=x,y=white] {data/utkface/arbitrariness_spread.dat};
\addplot [rblack,ultra thick,densely dashed] table[x=x,y=black] {data/utkface/arbitrariness_spread.dat};
\addplot [rasian,ultra thick,loosely dash dot dot] table[x=x,y=asian] {data/utkface/arbitrariness_spread.dat};
\addplot [rindian,ultra thick,densely dotted] table[x=x,y=indian] {data/utkface/arbitrariness_spread.dat};

% \legend{White, Black, Asian, Indian}

\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis} [width=0.37\linewidth,height=0.25\linewidth,ylabel={Ambiguity},ymin=0,ymax=0.3,xlabel={Race \vphantom{g}},enlarge x limits=0.25,xtick=data,ybar=0.5pt,bar width=8pt,axis y line*=left,axis x line*=bottom,symbolic x coords={{White},{Black},{Asian},{Indian}},ylabel near ticks,ylabel style={align=center, text width=4cm, font=\small},xlabel style={align=center, text width=4cm, font=\small},ticklabel style = {font=\small},
% legend pos=north west, legend columns=2,legend style={font=\small,at={(0.5,-0.4)},anchor=north}, 
title style={align=center, text width=5cm, font=\small},
title={\textbf{(b) Multiplicity Under Fairness Constraints\vphantom{g}}}
]

\addplot[style={fill=nocons,postaction={pattern=vertical lines}},draw=none
]
coordinates {({White},0.16301905717151456)
             ({Black},0.13922651933701657)
             ({Asian},0.2575250357653791)
             ({Indian},0.1608229426433915)
	     };

\addplot[style={fill=thres,postaction={pattern=horizontal lines}},draw=none
]
coordinates {({White},0.18505516549648948)
             ({Black},0.15359116022099448)
             ({Asian},0.2718168812589413)
             ({Indian},0.1770573566084788)
	     };

% \addplot[style={fill=rwhite},draw=none
% ]
% coordinates {({No Cons.},0.17301905717151456)
%              ({Thresh. Opt.},0.18505516549648948)
% 	     };
% \addplot[style={fill=rblack},draw=none
% ]
% coordinates {({No Cons.},0.13922651933701657)
%              ({Thresh. Opt.},0.15359116022099448)
% 	     };
% \addplot[style={fill=rasian},draw=none
% ]
% coordinates {({No Cons.},0.2675250357653791)
%              ({Thresh. Opt.},0.2718168812589413)
% 	     };
% \addplot[style={fill=rindian},draw=none
% ]
% coordinates {({No Cons.},0.1708229426433915)
%              ({Thresh. Opt.},0.1770573566084788)
% 	     };

% \legend{White, Black, Asian, Indian}

\end{axis}
\end{tikzpicture}%
% \hspace{1em}
\raisebox{3.3em}{
\begin{tikzpicture}
\begin{axis}[scale=0.01,
legend cell align={left},
hide axis,
% area legend,
xmin=0, xmax=1,
ymin=0, ymax=1,
legend columns=1,
legend style={font=\footnotesize,/tikz/every even column/.append style={column sep=0.1cm}}
]
\addlegendimage{ultra thick, rwhite}
\addlegendentry{Race: White};
\addlegendimage{ultra thick, rblack,densely dashed}
\addlegendentry{Race: Black};
\addlegendimage{ultra thick, rasian,loosely dash dot dot}
\addlegendentry{Race: Asian};
\addlegendimage{ultra thick, rindian,densely dotted}
\addlegendentry{Race: Indian};
\addlegendimage{ultra thick, white}
\addlegendentry{};
\addlegendimage{bar legend=nocons, nocons,fill=nocons,postaction={pattern=vertical lines}}
\addlegendentry{No Constraints};
\addlegendimage{bar legend=thres, thres,fill=thres,postaction={pattern=horizontal lines}}
\addlegendentry{Threshold Optimization};

\end{axis}
\end{tikzpicture}
}

==> figure_scripts/fig_arbitrariness_spread_jigsaw.tex <==
\begin{tikzpicture}
\begin{axis} [width=0.4\linewidth,height=0.25\linewidth,ylabel={Ambiguity},ymin=0,ymax=0.8,xlabel={Religion},enlarge x limits=0.2,xtick=data,ybar=0.5pt,bar width=8pt,axis y line*=left,axis x line*=bottom,symbolic x coords={{Budd.},{Christ.},{Hindu},{Jew.},{Muslim}},ylabel near ticks,ylabel style={align=center, text width=4cm, font=\small},
xlabel style={align=center, font=\small},ticklabel style = {font=\small},
% legend pos=north west, legend columns=2,legend style={font=\small,at={(0.5,-0.4)},anchor=north}, 
% title style={align=center, text width=5cm, font=\small},
% title={\textbf{(b)}}
]

\addplot[style={fill=reljig}
]
coordinates {({Budd.},0.4444444444444444)
             ({Christ.},0.29642058165548096)
             ({Hindu},0.5)
             ({Jew.},0.5897435897435898)
             ({Muslim},0.67601246105919)
	     };

\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis} [width=0.3\linewidth,height=0.25\linewidth,ymin=0,ymax=0.8,xlabel={Sexual Orientation \vphantom{g}},enlarge x limits=0.3,xtick=data,ybar=0.5pt,bar width=8pt,axis y line*=left,axis x line*=bottom,symbolic x coords={{Bi.},{Hetero.},{Homo.}},ylabel near ticks,ylabel style={align=center, text width=4cm, font=\small},
xlabel style={align=center, font=\small},
ticklabel style = {font=\small},
ytick=\empty,
% legend pos=north west, legend columns=2,legend style={font=\small,at={(0.5,-0.4)},anchor=north}, 
% title style={align=center, text width=5cm, font=\small},
% title={\textbf{(b)}}
]

\addplot[style={fill=sexjig}
]
coordinates {({Bi.},0.391304347826087)
             ({Hetero.},0.7096774193548387)
             ({Homo.},0.6225490196078431)
	     };

\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis} [width=0.3\linewidth,height=0.25\linewidth,ymin=0,ymax=0.8,xlabel={Gender Identity \vphantom{g}},enlarge x limits=0.3,xtick=data,ybar=0.5pt,bar width=8pt,axis y line*=left,axis x line*=bottom,symbolic x coords={{Male},{Female},{Trans.}},ylabel near ticks,ylabel style={align=center, text width=4cm, font=\small},
xlabel style={align=center, font=\small},
ticklabel style = {font=\small},
ytick=\empty,
% legend pos=north west, legend columns=2,legend style={font=\small,at={(0.5,-0.4)},anchor=north}, 
% title style={align=center, text width=5cm, font=\small},
% title={\textbf{(b)}}
]

\addplot[style={fill=genjig}
]
coordinates {({Male},0.3968253968253968)
             ({Female},0.4595635430038511)
             ({Trans.},0.5281553398058253)
	     };

\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis} [width=0.33\linewidth,height=0.25\linewidth,ymin=0,ymax=0.8,xlabel={Race \vphantom{g}},enlarge x limits=0.2,xtick=data,ybar=0.5pt,bar width=8pt,axis y line*=left,axis x line*=bottom,symbolic x coords={{Asian},{Black},{Latino},{White}},ylabel near ticks,ylabel style={align=center, text width=4cm, font=\small},xlabel style={align=center, font=\small},ticklabel style = {font=\small},
ytick=\empty,
% legend pos=north west, legend columns=2,legend style={font=\small,at={(0.5,-0.4)},anchor=north}, 
% title style={align=center, text width=5cm, font=\small},
% title={\textbf{(b)}}
]

\addplot[style={fill=racejig}
]
coordinates {({Asian},0.3805970149253731)
             ({Black},0.7786885245901639)
             ({Latino},0.45569620253164556)
             ({White},0.7574931880108992)
	     };

\end{axis}
\end{tikzpicture}

==> figure_scripts/fig_multiplicity_example.tex <==
\begin{tikzpicture}
\begin{axis} [width=0.37\linewidth,height=0.25\linewidth,yticklabel= {\pgfmathprintnumber\tick},ylabel={\# of Individuals (Test Set)},ymin=0,ymax=200,xmin=0.4,xmax=1.,xlabel={Self-Consistency (CDF)},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm, font=\small},xlabel style={align=center, text width=4cm, font=\small},
xtick={0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.},ticklabel style = {font=\small},
% legend pos=north west, legend columns=2,legend style={font=\small,at={(0.5,-0.4)},anchor=north}, 
title style={align=center, text width=5cm, font=\small},
title={\textbf{\vphantom{g}(a) Model Selection with Accuracy vs Both Accuracy and Fairness}}
]

\addplot [accsel,ultra thick] table[x=x,y=y] {data/credit/arbitrariness_spread_acc.dat};
\addplot [fairsel,ultra thick,densely dashed] table[x=x,y=y] {data/credit/arbitrariness_spread_fair.dat};

% \legend{White, Black, Asian, Indian}

\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis} [width=0.37\linewidth,height=0.25\linewidth,yticklabel= {\pgfmathprintnumber\tick},ylabel={\# of Individuals (Train Set)},ymin=0,ymax=800,xmin=0.4,xmax=1.,xlabel={Self-Consistency (CDF)},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm, font=\small},xlabel style={align=center, text width=4cm, font=\small},
xtick={0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.},ticklabel style = {font=\small},
% legend pos=north west, legend columns=2,legend style={font=\small,at={(0.5,-0.4)},anchor=north}, 
title style={align=center, text width=5cm, font=\small},
title={\textbf{\vphantom{g}(b) Predictive Multiplicity vs Multiplicity of Membership Inference}}
]

\addplot [predsel,ultra thick,loosely dash dot dot] table[x=x,y=y] {data/credit/arbitrariness_spread_pred.dat};
\addplot [miasel,ultra thick,densely dotted] table[x=x,y=y] {data/credit/arbitrariness_spread_mia.dat};

% \legend{White, Black, Asian, Indian}

\end{axis}
\end{tikzpicture}%
\raisebox{3.3em}{
\begin{tikzpicture}
\begin{axis}[scale=0.01,
legend cell align={left},
hide axis,
% area legend,
xmin=0, xmax=1,
ymin=0, ymax=1,
legend columns=1,
legend style={cells={align=left},font=\footnotesize,/tikz/every even column/.append style={column sep=0.1cm}}
]
\addlegendimage{ultra thick, accsel}
\addlegendentry{Performance Metric:\\ Accuracy};
\addlegendimage{ultra thick, fairsel,densely dashed}
\addlegendentry{Performance Metric:\\ Accuracy + Fairness};
\addlegendimage{ultra thick, white}
\addlegendentry{};
\addlegendimage{ultra thick, predsel,loosely dash dot dot}
\addlegendentry{Multiplicity Metric:\\ Model Predictions};
\addlegendimage{ultra thick, miasel,densely dotted}
\addlegendentry{Multiplicity Metric:\\ Membership Inference};

\end{axis}
\end{tikzpicture}
}

==> figure_scripts/fig_multiplicity_example_archived.tex <==
\centering
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=1 by 2,
        vertical sep=0pt
    },
    enlarge x limits=0.2,
    ybar=0.5pt,
    xtick=data,
    symbolic x coords={{$(0.4,0.5]$},{$(0.5,0.7]$},{$(0.7,0.9]$},{$(0.9,1.]$}},
    ylabel near ticks,
    xmin={$(0.4,0.5]$},
    xmax={$(0.9,1.]$},
    width=0.33\linewidth,
    scaled ticks=false,
    axis y line*=left
    ]

    \nextgroupplot[
      bar width=15pt,
      ylabel style={at={(-0.15, -0.2)}},
      ylabel={\# of Individuals},
      xtick=\empty,
      x axis line style={draw=none},
      axis y discontinuity=crunch,
      ymin=150,
      ymax=170,
      ytick={160,170},
      height=0.2\linewidth,
      % enlarge y limits=true
    ]

    \addplot[style={fill=lgreen},draw=none]
        coordinates {({$(0.9,1.]$},164)
	     };

    \nextgroupplot[
      bar width=15pt,
      xlabel={Self-Consistency},
      xtick=data,
      ymin=0,
      ymax=30,
      % enlarge y limits=true,
      axis x line*=bottom,
      height=0.25\linewidth
    ]

      \addplot[style={fill=lgreen},draw=none]
        coordinates {({$(0.4,0.5]$},3)
                    ({$(0.5,0.7]$},15)
                    ({$(0.7,0.9]$},18)
                    ({$(0.9,1.]$},164)
	     };

    \end{groupplot}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=1 by 2,
        vertical sep=0pt
    },
    enlarge x limits=0.25,
    ybar=0.5pt,
    xtick=data,
    symbolic x coords={{$0.4$},{$0.46$},{$0.66$},{$1.$}},
    ylabel near ticks,
    xmin={$0.4$},
    xmax={$1.$},
    width=0.33\linewidth,
    scaled ticks=false,
    axis y line*=left
    ]

    \nextgroupplot[
      bar width=15pt,
      % ylabel style={at={(-0.15, -0.2)}},
      % ylabel={\# of Individuals},
      xtick=\empty,
      ytick=\empty,
      x axis line style={draw=none},
      axis y discontinuity=crunch,
      ymin=150,
      ymax=170,
      % ytick={160,170},
      height=0.2\linewidth,
      % enlarge y limits=true
    ]

    \addplot[style={fill=lgreen},draw=none]
        coordinates {({$1.$},168)
	     };

    \nextgroupplot[
      bar width=15pt,
      xlabel={Self-Consistency},
      xtick=data,
      ytick=\empty,
      ymin=0,
      ymax=30,
      % enlarge y limits=true,
      axis x line*=bottom,
      height=0.25\linewidth
    ]

      \addplot[style={fill=lgreen},draw=none]
        coordinates {({$0.4$},3)
                    ({$0.46$},8)
                    ({$0.66$},21)
                    ({$1.$},168)
	     };

    \end{groupplot}
\end{tikzpicture}%
\hfill
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=1 by 2,
        vertical sep=0pt
    },
    enlarge x limits=0.25,
    ybar=0.5pt,
    xtick=data,
    symbolic x coords={{$0.4$},{$0.46$},{$0.66$},{$1.$}},
    ylabel near ticks,
    xmin={$0.4$},
    xmax={$1.$},
    width=0.33\linewidth,
    scaled ticks=false,
    axis y line*=left
    ]

    \nextgroupplot[
      bar width=15pt,
      ylabel style={at={(-0.15, -0.2)}},
      ylabel={\# of Individuals},
      xtick=\empty,
      x axis line style={draw=none},
      axis y discontinuity=crunch,
      ymin=520,
      ymax=600,
      ytick={550,600},
      height=0.2\linewidth,
      % enlarge y limits=true
    ]

    \addplot[style={fill=lgreen},draw=none]
        coordinates {({$1.$},680)
	     };

    \nextgroupplot[
      bar width=15pt,
      xlabel={Self-Consistency},
      xtick=data,
      ymin=0,
      ymax=120,
      % enlarge y limits=true,
      axis x line*=bottom,
      height=0.25\linewidth
    ]

      \addplot[style={fill=lgreen},draw=none]
        coordinates {({$0.4$},17)
                    ({$0.46$},46)
                    ({$0.66$},57)
                    ({$1.$},680)
	     };

    \end{groupplot}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=1 by 2,
        vertical sep=0pt
    },
    enlarge x limits=0.25,
    ybar=0.5pt,
    xtick=data,
    symbolic x coords={{$0.4$},{$0.46$},{$0.66$},{$1.$}},
    ylabel near ticks,
    xmin={$0.4$},
    xmax={$1.$},
    width=0.33\linewidth,
    scaled ticks=false,
    axis y line*=left
    ]

    \nextgroupplot[
      bar width=15pt,
      ylabel style={at={(-0.15, -0.2)}},
      ylabel={\# of Individuals},
      xtick=\empty,
      x axis line style={draw=none},
      axis y discontinuity=crunch,
      ymin=520,
      ymax=600,
      ytick={550,600},
      height=0.2\linewidth,
      % enlarge y limits=true
    ]

    \addplot[style={fill=lgreen},draw=none]
        coordinates {({$1.$},592)
	     };

    \nextgroupplot[
      bar width=15pt,
      xlabel={Self-Consistency},
      xtick=data,
      ymin=0,
      ymax=120,
      % enlarge y limits=true,
      axis x line*=bottom,
      height=0.25\linewidth
    ]

      \addplot[style={fill=lgreen},draw=none]
        coordinates {({$0.4$},22)
                    ({$0.46$},79)
                    ({$0.66$},107)
                    ({$1.$},592)
	     };

    \end{groupplot}
\end{tikzpicture}%

==> sections/discussion.tex <==

In our study, we compared two different types of Large Language Models: BERT and autoregressive models such as Falcon, Llama 2, and GPT-2, which differ in structure and the methods used to achieve results. The development of these models has increasingly focused on optimizing their capabilities to understand and generate human-like text. However, our comparative analysis leads us to hypothesize that the efficacy of these models in bias mitigation and reasoning tasks is heavily dependent on the nature and quality of their training data. We believe this underscores the potential impact of data diversity and curation on model behavior and performance, although further evidence is needed to confirm these observations.

\begin{enumerate}

\item \textbf{Impact of Data Quality and Composition:} BERT' lower socioeconomic biases is primarily due to its reliance on cleaner, more structured data sources, namely BookCorpus and English Wikipedia. These sources provide a well-curated foundation that reduces the likelihood of learning and propagating biases found in less controlled environments. In contrast, GPT-2 are trained on extensive but unfiltered datasets like WebText, which capture a wider array of internet discourse but also its inherent biases. This is evident from the model documentation provided by OpenAI, highlighting concerns regarding the propagation of stereotypes and the need for careful deployment in bias-sensitive applications. While data cleaning strategies and such as RefinedWeb for Falcon might help obtain better results for reducing direct biases \cite{he2023exploring}, they are not enough to compensate the capability of new models to reverberate these biases in other aspects were complex link exist. Moreover, our study emphasize once again the importance of controlling and cleaning dataset when training model because of the difficulty to control and understand all biases that could be implied in the future even with mitigation strategies. Especially when the specificity of these strategies are not released to research and hidden under wording as helpfulness or harmless. 

\item \textbf{Training Data Diversity and Model Generalization:} The diversity in training datasets, as seen with Falcon and Llama 2, prepares models to handle a broader range of linguistic styles and contexts. This is beneficial for generalization across different tasks. However, the challenge remains in balancing this diversity with the need to control for quality and bias, which is critical for ensuring that models do not amplify harmful stereotypes or misinformation.

\item \textbf{Instruction-Based Design and Enhanced Reasoning:} LLama 2 and Falcon, designed to be more instruction-sensitive, demonstrate an advanced capacity for detailed reasoning . With 

as shown in the case studies from Figure !!!! in the appendix. These models, through their diversified training that likely includes conversational and contextual data, excel in generating nuanced responses. This capability is crucial for applications requiring detailed explanatory outputs and where understanding the context of queries is essential. However, the detailed reasoning ability does not necessarily equate to fairness or lesser bias, as highlighted by their performance relative to simpler models like BERT in certain contexts.

\end{enumerate}



